SLM Lab: A Comprehensive Benchmark and Modular Software Framework for Reproducible Deep Reinforcement Learning

We introduce SLM Lab, a software framework for reproducible reinforcement learning (RL) research. SLM Lab implements a number of popular RL algorithms, provides synchronous and asynchronous parallel experiment execution, hyperparameter search, and result analysis. RL algorithms in SLM Lab are implemented in a modular way such that differences in algorithm performance can be confidently ascribed to differences between algorithms, not between implementations. In this work we present the design choices behind SLM Lab and use it to produce a comprehensive single-codebase RL algorithm benchmark. In addition, as a consequence of SLM Lab's modular design, we introduce and evaluate a discrete-action variant of the Soft Actor-Critic algorithm (Haarnoja et al., 2018) and a hybrid synchronous/asynchronous training method for RL agents.

==> library_comp_notes.tex <==
% \paragraph{Quotes from whitepapers}

% "Reliable and reproducible: A reliable framework is one that is demonstrably correct; in software engineering this is typically achieved via tests. A reproducible framework is one that facilitates the regeneration of published statistics, and makes novel scientific contributions easily shareable with the community."\citep{dopamine}

% "we propose ELF, an Extensive, Lightweight and Flexible platform
% for fundamental reinforcement learning research" \citep{facebook-elf}

% "We argue for distributing RL components in a composable way
% by adapting algorithms for top-down hierarchical control, thereby encapsulating parallelism and resource requirements within short-running compute tasks" \citep{ray-rllib}

% "The purpose of OpenSpiel is to promote general multiagent reinforcement learning across many different game types." \citep{openspiel} 
% Keep it simple. Keep it light. \citep{openspiel}

% "MAgent, a platform to support research and development of many-agent reinforcement learning. Unlike previous research platforms on single or multi-agent reinforcement learning, MAgent focuses on supporting the tasks and the applications that require hundreds to millions of agents." \citep{magent}

% "Models should be runnable from the configuration files that are easy to store in version control, generate automatically and diff. Codebase should be generic and do not contain any of the model hyperparameters. Unless user intervenes, it should be obvious which model was run with which hyperparameters and what output it gave." \citep{vel}

% "Reaver is a modular deep reinforcement learning framework with a focus on various StarCraft II based tasks" \citep{reaver}

% citations for rl libraries
% ray-rllib \citep{ray-rllib}, Softlearning \citep{softlearn}, ChainerRL \citep{chainer, chainerrl}, OpenSpiel \citep{openspiel}, TRFL \citep{deepmind-trfl}, ELF \citep{facebook-elf}, Horizon \citep{facebook-horizon}, garage \citep{garage}, Dopamine \citep{dopamine}, TF-Agents \citep{TFAgents}, MAgent \citep{magent}, coach \citep{coach}, Baselines \citep{baselines}, a2c-ppo-acktr-gail \citep{kostrikov}, pytorch-rl \citep{pytorch-rl}, RLgraph \citep{rlgraph}, RLKit \citep{rlkit}, Stable Baselines \citep{stable-baselines}, TensorForce \citep{tensorforce}, Unity ML Agents \citep{unity-ml}, vel \citep{vel}, reaver \citep{reaver}

Config notes

a2c-ppo-acktr-gail: has a get args file - same for all algorithms

baselines: has just an atari defaults for dqn only with a few params

chainerRL - has a lot of examples. the hyperparams are specified here.

coach: https://github.com/NervanaSystems/coach/tree/master/rl_coach/presets
extensive examples, but split between multiple files

DeepRL: set of examples here, but network arch missing
https://github.com/ShangtongZhang/DeepRL/blob/f2097912b76d1d66da2495ad2afe74fd120b0fe0/examples.py
network specified here e.g.
https://github.com/google/dopamine/blob/master/dopamine/discrete_domains/atari_lib.py

Keras-RL:
some examples which can be run directly (e.g. dqn atari, dqn cartpole, ddpq mujoco). The config is specified here but no separate file.

rlpyt:
environment and training params specified in examples file. Models specified in a separate file e.g. atari_dqn_model.py epsilon decay in the episilon greedy agent. Other params e.g discount prioritized replay etc in agent class.

ELF:

Horizon: uses config file for tests - most similar so far
https://github.com/facebookresearch/Horizon/blob/master/ml/rl/test/configs/discrete_dqn_pocman_v0.json
Lots of examples for testing, does seem to be able to include everything including network arch
https://github.com/facebookresearch/Horizon/blob/43997325396bf0dbd4ad148649120a32052182de/ml/rl/test/gym/discrete_dqn_lunarlander_v2.json

reaver: gin files
https://github.com/inoryy/reaver/blob/master/reaver/configs/atari/base.gin
models / policies are specified elsewhere. No env info in these files e.g. num training steps, num envs

RLgraph: everything is in - most similar.
https://github.com/rlgraph/rlgraph/blob/master/examples/configs/apex_pong.json

RLLib: mixed - what is included varies by file
partial, no training length, network arch, lr etc
https://github.com/ray-project/ray/blob/master/rllib/tuned_examples/atari-ppo.yaml
no lr or training length
https://github.com/ray-project/ray/blob/master/rllib/tuned_examples/pong-a3c.yaml

Softlearn: variant.py file
https://github.com/rail-berkeley/softlearning/blob/59f9ad357b11b973b9c64dcfeb7cf7b856bbae91/examples/development/variants.py

Stable baselines: no spec file, just run files
https://github.com/hill-a/stable-baselines/blob/master/stable_baselines/deepq/experiments/run_atari.py

vel: everything except network arch
https://github.com/MillionIntegrals/vel/blob/master/examples-configs/rl/atari/dqn/breakout_dueling_ddqn_prioritized.yaml


==> limbo.tex <==
Modularity limbo

Example: AC extends REINFORCE, PPO extends AC. Uses class inheritance. Example PPO: algorithm says just the loss function and training loop changes, and the code actually shows that by extending AC and adding these two components, and not more.

DQN extensions are implemented as components that can be toggled on top of base DQN class.

Example: SAC is the current state-of-the-art algorithm for continuous control tasks. It is an Actor-Critic algorithm, so it can naturally be implemented as an extension to the corresponding \verb|ActorCritic| class. 

It was only necessary to implement the components of SAC that are different from A2C, namely the $Q$-networks, loss functions, and training loop. First, SAC contains a policy network and two $Q$ networks with their respective target networks. The $Q$ networks have a special architecture and are easily declared using the Network API in SLM Lab. Second, the algorithm computes three loss functions --- a policy loss, $Q$-function loss, and a temperature loss, all of which are implemented in a manner that directly corresponds to their respective theoretical forms by making use of utility functions available. Third, the training loop is straightforward to implement once the loss functions are defined.

SAC was implemented after the Actor-Critic implementation in SLM-Lab was finished and well-tested. Consequently, a complex algorithm became straightforward to implement and debug. The implementation is also short --- only ~375 additional lines of code were required to implement SAC; 250 lines for the algorithm component, and 125 lines for the $Q$-network.

Finally, using the reparametrizable discrete distribution known as Gumbel-Softmax (TODO cite Concrete distribution and Eric Jang), SAC was easily extended to discrete action spaces.

\todo[inline]{Compare SAC implementation length with other libraries}

Implementation speed: just an extension. Safety: reuse well-tested components.

Shared API: Hogwild can be applied to all algorithms in SLM Lab by just toggling it on with a flag.

useful abstractions and modularization help understand the algorithms better by breaking it into simpler chunks.


Two examples:

1. Hybrid of synchronous and asynchronous parallelization is possible and was not deliberately implemented, but emerged from the design. Given a desired quantity of parallelization, e.g. 128 workers, the workers can be split between sync and async. For example 16 asynchronous workers, each with 8 synchronous workers (implemented as a vector environment).

One benefit is to match the resources available. E.g. vector environment (sync) is cheap but requires a single thread so there is a limit (?). Async requires a separate process. Example of SAC training 100M frames on a single machine in xx days using 32 sync processes each with xx vector environments. A second benefit is that it may lead to better results. 

2. SAC + PER naturally arises once SAC implemented.

\todo[inline]{Note sync and async training can be mixed. Haven't seen this anywhere else}

Component reuse to minimize implementation differences, to not introduce more discrepancies other than true differences between algorithms. This allows for fairer comparison.

% \subsubsection{Case Study: Implementing SAC}

% \mcc{I'm not 100\% sold on this section, but it might be good to include if we make it a bit more succinct.}
% \lhg{Potentially shorten and fold into modularity / implementation lessons section}

% Showcase design benefits connecting to the points before. E.g. minimal differences allows for fairer comparison. Connect back to design principles.

% To showcase the design benefits of SLM Lab, we provide an anecdote on how we recently implemented Soft Actor-Critic (SAC) --- a state-of-the-art model-free RL algorithm\cite{sac2} that is fairly involved.

% % LG: moved the next three paragraphs to modularity sections
% Since SAC is an Actor-Critic algorithm, we start by extending the existing \verb|ActorCritic| class for the A2C algorithm in SLM Lab to reuse methods. All other components such as replay memory, data preprocessing, and environment interaction make use of existing components in SLM Lab. This allows for quick and reliable implementation due to many reusing of well-tested components.

% Specifically, we only implement the components of SAC that are different from A2C, namely the networks, loss functions, and training loop. First, SAC contains a policy network and two $Q$ networks with their respective target networks. These are easily declared using the Network API in SLM Lab. Second, the algorithm computes three loss functions --- a policy loss, $Q$-function loss, and a temperature loss, all of which are implemented in a clean manner that directly corresponds to their respective theoretical forms by making use of utility functions available. Third, the training loop is straightforward to implement once the loss functions are defined. 

% Although the formulation of SAC is generic to both continuous and discrete actions, the authors have only provided implementation details for the continuous case. To our knowledge, we have not seen a discrete implementation of SAC with an accompanying benchmark. Theoretically, the discrete case is only different from the continuous case by its type of action policy distribution. However, the policy loss requires the policy distribution to be reparametrizable, but many discrete distributions are not. We suspect this is the main challenge for its implementation. Fortunately, SLM Lab includes a reparametrizable discrete distribution known as Gumbel-Softmax (cite Concrete distribution and Eric Jang), so we simply use it for the discrete case, and discrete SAC is implemented. We provide the first known discrete benchmark for SAC.

% The full SAC implementation in SLM Lab is contained within a single file located at \url{https://github.com/kengz/SLM-Lab/blob/master/slm_lab/agent/algorithm/sac.py}. The concise implementation was accompanied a basic benchmark before being merged into SLM Lab. See the Pull Request at \url{https://github.com/kengz/SLM-Lab/pull/402}.

% Additionally, due to easy composability of components in SLM Lab, we can easily use SAC with PER, and use Asynchronous SAC via Hogwild (same spirit as A3C). We also provide the first known benchmark for SAC+PER and Async-SAC.

% \todo[inline]{Add note about lab API / algorithm framework helping to organize code and implementation when new code needs to be written - this makes it more manageable than implementing from scratch}
% \todo[inline]{Discrete SAC Atari benchmark}
% \todo[inline]{SAC+PER benchmark}
% \todo[inline]{Async-SAC benchmark}
% \paragraph{Parallelism} Almost 

% \parallelism{hyperparameter optimization} Very few libraries include an automatic hyperparameter tuning feature. The exception is Stable Baselines \citep{stable-baselines} and Tensorforce \citep{tensorforce}.

% \paragraph{Plots}
% \todo[inline]{Use a comparison table for main features vs other frameworks}
% \todo[inline]{List other frameworks in appendix}

% See https://github.com/kengz/awesome-deep-rl

% \lhg{Dopamine uses class inheritance for all its algos}

% Other frameworks have bits and pieces, only implement a subset of algos, or lack analysis framework, lack organization.

% None of them have a the reproducibility workflow of SLM Lab: fully exposed spec with plus git SHA.
% SLM Lab also has more component sharing and reuse than the others, thereby minimizing the algo differences. Uses class extension, whereas other implementations are one-off adhoc, self-contained code without much component sharing or reuse.

% One way to structure this section could be around a set of questions which compare the libraries amongst themselves and SLM-Lab. Note that the library review still needs to be completed.

% \keng{relate back to the things we highlight in feature table, would nicely correspond and guide people.}
% \keng{Missed some big libraries below. Check the awesome-rl-list again.}


% \begin{enumerate}
%     \item How many algorithms are implemented? Does a library aim to be comprehensive or specialize in a particular subset. Examples of comprehensive libraries include garage (formerly ray-rllib), OpenAI Baselines, ChainerRL, DeepRL (and what others?). Examples of specialist libraries are Berkeley Softlearning, ELF (focuses on AlphaGo / AlphaZero) (and what others?). SLM-Lab implements a broad range of algorithms, but is not the most comprehensive. garage, ChainerRL have more.
%     \item Parallelized training. SLM Lab is the only one to seamlessly mix synchronous and asynchronous training. This fell out of the design. There was no need to deliberately added, it was naturally possible after the two features had been implemented separately.
%     \item What benchmarks are provided with the libraries? This is very mixed. OpenAI baselines and garage (ray-rllib) appear to be the most comprehensive here. OpenAI baselines provides a detailed benchmark on Atari Games for many algorithms (PPO, deepQ (Dueling Double DQN + PER - to check), acktr, acer, trpo, a2c) and Mujoco for trpo and ppo. Final rewards and learning curves are provided for both. Additionally, more detail on Atari games in other parts of the repo. garage (ray-rllib) reports results and learning curves for a wide range of algorithms on 4 Atari games. Other libraries don't report any results, e.g. ChainerRL (what others?) No benchmarks on SAC in any library (to check). How old are the benchmarks?
%     \item How easy are results to reproduce?
%     \begin{enumerate}
%         \item \textbf{config} In most libraries (to check) the hyperparameter configuration is through command line arguments and we have to assume that the default configuration is the best. How many libraries log the hyperparameters when an experiment is run? Are there any? The closest to SLM-Lab appears to be garage (ray-rllib) which defines a set of default configurations for many algorithms in yaml files (to check if these are saved when running an experiment). Reproducibility does not appear to be a high priority for many of the libraries - SLM-Lab is the only library (to check) that contains and sufficient information in the log directory to fully reproduce an experiment. Additionally SLM-Lab emphasizes reproducibility as shown by the command that will re-run an experiment in a single line given the path to the relevant spec in the experiment data folder.
%         \item \textbf{experiment replication with multiple random seeds} Only OpenAI baselines (to check) includes experiment replication in a single training run with different random seeds by default. This is built into the heart of SLM-Lab, and results are by default reported averaging over multiple random seeds.
%     \end{enumerate}
%     \item hyperparameter search: SLM-Lab focuses significantly on reducing the time and effort required to do hyperparameter search. No other library (to check) provides this feature at all, let alone the ability to search over any possible hyperparameter including environment features. 
%     \item How much experiment analysis is carried out by default. Experiment log data - SLM-Lab logs a large number of metrics during training (reward, loss, fps, entropy, exploration ...) and automatically generates plots. No library (to check) does this as extensively. OpenAI baselines has a tutorial on plotting results using experiment data, but they are not generated automatically. SLM-Lab experiment PR also appears to be unique. To check other libraries.
%     \item Software design. How integrated are the different algorithm implementations? Is class inheritance used? How extensively is the library tested? SLM-Lab makes extensive use of class inheritance to share common code between algorithms. Other libraries are positioned along a spectrum from being a collection of independently implemented algorithms (give e.g.s) to partial code sharing of common components such as (todo), but with little or no class inheritance (give e.g.s) How many PPO and SAC implementations inherit from A2C? And how many A2C inherit from REINFORCE? Design principles for SLM-Lab appear to be quite different to all the other libraries in its emphasis on code re-use and unit testing.
% \end{enumerate}

% \keng{in software design, add the effect of modularity and reuse (instead of just stating it without a purpose): minimize differences among algorithms for fairer comparisons. fold into class diagram, can also clearly see the point in the diagram.}

% To summarize - SLM-Lab is most different in its emphasis on reproducibility - a large part of the lab is designed to support this, hyperparameter search, and software design. The analysis module is richer than others available. The benchmarks are at the least comparable with the most extensive benchmarks in other libraries. SLM-Lab does not stand out in terms of the number of implemented algorithms.

% Somehow also mention Benchmark, and only some of those provide as "proofs" of implementation. the RL list also has a list of them but sadly it's small.

% \lhg{How to select libraries?}
% \keng{At this rate we might need to rotate into a full-page horizontal table. Unless if we picked the top 4 or 5 only. Also not sure if there's much value to people in a super comprehensive comparison, in that the comparison table itself is not a contribution, but good reference to have.}


